Rethinking STS and NLI in Large Language Models

Recent years have seen the rise of large language models (LLMs), where practitioners use task-specific prompts; this was shown to be effective for a variety of tasks. However, when applied to semantic textual similarity (STS) and natural language inference (NLI), the effectiveness of LLMs turns out to be limited by low-resource domain accuracy, model overconfidence, and difficulty to capture the disagreements between human judgements. With this in mind, here we try to rethink STS and NLI in the era of LLMs. We first evaluate the performance of STS and NLI in the clinical/biomedical domain, and then we assess LLMs' predictive confidence and their capability of capturing collective human opinions. We find that these old problems are still to be properly addressed in the era of LLMs.

==> literature.tex <==
\section{Related Work}
\paragraph{Chain of Thought}
Scaling up model size alone has not proved sufficient for achieving high performance on challenging tasks, such as tasks requiring reasoning.
Chain of thought prompting was proposed to unlock the reasoning ability of large language models.
It is superior to standard prompting (only few-shot examplars with input and answer) across arithmetic reasoning, commonsense and symbolic reasoning tasks.
Analysis over arithmetic reasoning demonstrated its robustness against variations of exemplars' annotators, independently-written chains of thought, different exemplars, various language models, different exemplar orders and varying numbers of exemplars~\citep{wei2022chain}.


There are some interesting findings and take-away points:
1. chain-of-thought prompting does not positively impact performance for small models, and only yields performance gains when used with models of $\sim$100B parameters.
Models of smaller scale produced fluent but illogical chains of thought, leading to lower performance than standard prompting.
2. chain-of-thought prompting has larger performance gains for more-complicated problems. On the easiest arithmetic data set that requires a single step to solve, performance improvements were either negative or very small.
3. With chain-of-thought prompting, in out-of-domain symbolic reasoning, language models achieve upward scaling curves though performance is lower than in the in-domain setting.
It is important to see the trend of upward curve, instead of toward stable, it implies locked potential if we continue to draw this curve.

% I like figures and presentation manner of this paper, clear, natural, easy to follow and tell the story from an intuition then to a hypothesis, then to verify and speculate. 
% I like this paper.

How about the performance using standard prompting over STS and NLI?
How to unlock semantic reasoning ability of large language models over STS and NLI models is our question.


\paragraph{NLU analysis using davinci}
\citet{chen2023howrobust} performed a comprehensive experimental analysis of GPT \textit{text-davinci} series,  exploring its robustness using 21 datasets over 9 natural language understanding (NLU) tasks.
Analysis shows that \textit{text-davinci} still encounters significant robustness degradation, such as its average performance dropping by up to 35.74\% and 43.59\% in natural language inference and sentiment analysis tasks, respectively.
What does this finding imply? Why does \textit{text-davinci} perform poorly in NLI and SA?

We attempt to check results over sentence relationship tasks, including NLI and paraphrase detection.
Seemingly, they add perturbations to the original text to examine the robustness of models, while unfortunately there isn't detailed descriptions of what perturbations means over each results tables.
This makes it difficult to follow and analyse experiment results.

We are interested in NLI and STS across domains, particularly biomedical and clinical.
We wonder (1) how do LLMs perform over NLI and STS, does it face the same challenge stemming from long-tail knowledge? (2) can it perceive the labelling uncertainty due to subjectivity for STS and NLI? (3) can it capture the collective human opinions, the full distribution? (4) can it assign personalised labels given the characteristics of a rater, furthermore, can it be used to collect crowdsourcing-like data? How about the quality? if so, we don't need to collect by employing so many annotators. 

After answering these questions, it may give us some hints what the most powerful model can do? how well it does the task, what is the limitations, for NLI and STS, especially in terms of uncertainty-aware modelling, how can future work continue to do.


This paper also want to evaluate robustness, however, compared with section 3.4 of chain of thought, it is too dry, and not that insightful.
Presentation by Tables is also not intuitive compared with bar chart and curves.
Tables or some other not remarkable results can all be put into Appendix, then presenting results supporting findings in the main body content by intuitive figures, bars and curves. 


\paragraph{Evaluation NLP tasks by ChatGPT}

\citet{zhong2023can} has found ChatGPT shows significantly better performance on inference tasks, has comparable performance on sentiment analysis and question-answering tasks, and has poor performance on paraphrase and similarity tasks when compared with 4 representative BERT-based fine-tuning methods.
% Any insights or analysis on why it perform poorly on paraphrase and similarity tasks?


\citet{luo2023chatgpt} explored the ability of ChatGPT to assess the factual consistency in abstractive summarisation by zero-shot and zero-shot with chain of thought, evaluating whether the generated summaries containing information that is not entailed by the source article1 with input documents.
They applied three tasks: entailment inference to estimate whether all information in the summary is supported by the article by answer (yes/no), summary ranking to choose consistent one over two candidate summaries given the source document, and consistency rating task to assign a consistency score in range of 0-10.
It showed that ChatGPT outperformed previous factuality metrics over 6/9 datasets, empirically demonstrating the great potential of ChatGPT as a good factual inconsistency evaluator.
% Section 2.2 in this paper presents the latest work of chatgpt for nlp tasks


\paragraph{Annotate NLI/STS data by PLM/LLM}
% Can machines learn to understand instructions as well?
In 2020, \citet{efrat2020turktest} examined a pre-trained langauge model (PLM) ability to follow natural language instructions of varying complexity, ranging from simple tasks (retrieving the nth word of a sentence), to ones that require creativity, such as generating examples for SNLI and SQuAD in place of human intelligence workers (\textit{turkers}). 
Despite the lenient evaluation, GPT-2 performs poorly across all tasks.
In 2021, \citet{schick-schutze-2021-generating} leveraged generative abilities of large and high-performing PLMs (GPT2-XL) to generate entire datasets of labelled STS pairs from scratch.
To assess the quality of the generated datasets, they use them to train Sentence-RoBERTa.
As an unsupervised method, over several STS datasets, it outperforms baselines such as Sentence-RoBERTa fine-tuned on NLI data and InferSent.
This work demonstrated the potential of LLMs to generate labelled datasets for STS.
It might be noisy but helpful to improve the quality of sentence embedding.
This inspires us to train domain-agnostic sentence embeddings utilising data extracted from larger language models, such as ChatGPT.


\paragraph{Other findings}
Bias (high word overlap of entailment pairs) in NLI annotation may impact the robustness of supervised NLI models.
Simply appending a neutral non-sense sentence such as \textit{not false is true} to hypothesis sentences significantly impact supervised NLI models~\citep{bhullar2023augmenting}.
\citet{wallace-etal-2019-universal} proposed universal triggers for attacking and analysing NLP tasks, such as NLI.
This may useful when you want to attack existing STS/NLI models, to know their weaknesses.



\paragraph{Clinical and Biomedical Domains}
\citet{singhal2023large} assess LLM's (PaLM) potential in medicine through the answering of medical questions.
They first introduce MultiMedQA, a benchmark combining six existing medical question answering datasets and a new collected dataset of medical questions searched online, HealthSearchQA. 
Using prompt original PaLM, instruction-tuned Flan-PaLM and instruction-prompt-tuned Med-PaLM, they evaluate on MultiMedQA.
Using a combination of prompting strategies (few-shot, chain of thought and self-consistency), Flan-PaLM achieves state-of-the-art accuracy on every MultiMedQA multiple-choice dataset (MedQA, MedMCQA, PubMedQA and Measuring Massive Multitask Language Understanding (MMLU) clinical topics).

In addition to the accuracy of multi-choise questions, they propose a human evaluation framework for model answers along multiple axes including factuality, comprehension, reasoning, possible harm and bias. 
Specifically, they ask a panel of clinician and layer users to evaluate the responses for 140 examples on the axes mentioned above.
There are three major findings:
1. model scaling improves performance.
2. instruction tuning is very useful.
3. they introduce instruction prompt tuning, a parameter-efficient approach for aligning LLMs to new domains using a few exemplars. The resulting model, Med-PaLM, performs encouragingly, but remains inferior to clinicians.

They find chain of thought hurts performance, this is consistent with our findings.


\subsection{In-context learning}
What is in-context learning? 
Models are given a few exemplars of input–label pairs as part of the prompt before performing the task on an unseen example.
\citet{min-etal-2022-rethinking} showed the surprising result that using random ground-truth labels in exemplars barely hurts performance, suggesting that models primarily rely on semantic prior knowledge, and the performance is instead mainly driven by the label space, distribution of input text, and overall format of the sequence.

\citet{wei2023llmdifferently} propose research question: how is in-context learning (ICL) in language models affected by semantic priors versus input–label mappings?
They investigate two settings: ICL with flipped labels and ICL with semantically-unrelated labels.
They assume that if language models can predict flipped labels correctly, they override prior knowledge, if they predict irrelevant labels correctly, they learn patterns from exemplars in the prompt, instead of only depending on prior knowledge.

Experiments on ICL with flipped labels show that overriding semantic priors is an emergent ability of model scale. While small language models ignore flipped labels presented in-context and thus rely primarily on semantic priors from pretraining, large models can override semantic priors when presented with in-context exemplars that contradict priors, despite the stronger semantic priors that larger models may hold. 

Study on semantically-unrelated label ICL (SUL-ICL), in which labels are semantically unrelated to their inputs (e.g., foo/bar instead of negative/positive), thereby forcing language models to learn the input–label mappings shown in in-context exemplars in order to perform the task. 
The ability to do SUL-ICL also emerges primarily with scale, and large-enough language models can even perform linear classification in a SUL-ICL setting. 
Experiments on ICL with flipped labels using instruction-tuned models shows that they perform worse than the base model. This trend suggests that instruction tuning strengthens both the use of semantic priors and the capacity to learn input–label mappings, but more of the former.
% \citet{wei2022chain} 

\citet{wei2023symboltuning} further propose another tuning strategy --- symbol tuning, compensating instruction tuning weakness that models are not forced to learn to use the exemplars because the task is redundantly defined in the evaluation example via instructions and natural language labels.

In in-context learning, depending on with/without instructions and using natural language relevant labels or irrelevant labels (symbol), we have four settings.
1. relevant label, instruction
2. relevant label, no instruction (naive few-shot prompt)
3. irrelevant label, instruction (equal to zero-shot but irrelevant labels may confuse models)
4. irrelevant label. no instruction

Symbol tuning leverages the intuition that when a model cannot use instructions or natural language labels to figure out a task, it must instead do so by learning the input–label mappings.
It forces model to learn mapping function between input and labels, as it cannot depends on priors.
Because symbol tuning teaches the model to reason over the in-context exemplars, symbol-tuned models should have much better performance on unseen tasks that require reasoning between in-context exemplars and their labels.

Experiments show that tuning 1k-2k steps over >16\% symbol data (the proportion of symbol data among all instruction tuning data) comparable results with tuning 10k steps and fully symbol data. 
However, for non-trivial task like following flipped-labels, symbol-tuning data is much more impactful for succeeding in flipped-label settings. We find that there is a strong correlation between a higher mixture of symbol-tuning data and a model’s ability to follow flipped labels.
Overall, symbol-tuned models show large improvements in following flipped-labels.



\section{Proposal}
what's the current findings and progress of in-context learning in STS and NLI?
Research questions you expect to know the answer: 
-- how to estimate personalised individual judgement for subjective ratings tasks, such as STS, SA? 
-- How reliable is ChatGPT on STS and NLI Estimation over Collective Human Opinions
    - Can chatgpt imitate individual rating given proper prompt?
    - How it performs?
    - Can a collection of estimated individual rating fit the empirical score distribution?
    - Does this imply the potential for ChatGPT to label traditional simple NLU tasks, replacing previous crowdsourcing, what is the advantage, limitations and concerns?
    - How about it performs in knowledge-rich domains, such as clinical and biomedical, what's the bottleneck and concerns here?
    - Extend to subjective NLI task, can it perform well?
    - Discussion, what do these findings suggest? What's the direction for future NLI, STS and SA tasks? What aspects LLMs can help? What aspects it can not? What should researchers go in the next step for these tasks?
    In terms of trustworthiness and robustness, what kind of attack we can conduct to know the weaknesses of current methods, just as machine-generated detection methods, we know that it is vulnerable to self-prompt edit and bias to non-native speaker text. 
    What's the limitations for current STS and NLI methods? Can LLMs address? How to?

-- Rethink STS and NLI under LLMs
    - what's the performance of STS and NLI under LLMs, what's the advantage and what's the limitation?
    - Is low-resource domain and language still the challenge? Any boosts or any declines? Why? How to fix it?
    - Any method can consistently output reliable and robust outputs based on LLMs
    - How will STS and NLI development in LLM era? Will they still be meaningful tasks? What makes them still meaningful, and what aspects have been out-of-date that requires update?


Steps:
1. No matter in which direction, we need first know the progress of STS and NLI after LLMs, how other researchers in this direction think about? What are they investigating? What is the current discussion?
2. summarise includes information: 
    - what's the current performance? 
    - Why it is good? Why it is bad? 
    - Is it robust? robust in which perspective? 
    - How did others detect its robustness? 
    - Is the output reliable? How others define reliability? 
    - How did they design to verify or investigate? 
    - How other research go in the direction of reliability?
3. For task subjectivity, we estimate the full population distribution by estimating individual ratings, how did other research do?

After reading related work and write the storyline. Design experiments to act.


==> section/discussion.tex <==
\section{Discussion}
\textbf{What does LLMs' output represent?}
For STS and NLI, we find the prediction reflects an average opinion.
Even if explicitly asking LLM to make personalised rating based on the given role, or to make estimation under domain-specific context and knowledge, the output does not change as expected, but fluctuate around the average opinion.
Put differently, the predictive uncertainty caused by changing system roles and contexts is almost similar to the uncertainty from random sampling under a completely same setting including prompts, system role, parameters and data.


\textbf{Is exploring STS still meaningful under LLMs? Why? What might be the future direction?}


pros and cons
LLMs+in-context learning by prompts vs. PLM+fine-tuning

future directions for STS and NLI modelling in low-resource domain and uncertainty-aware estimation

a preliminary experiment to test or evaluate the core direction idea, provide the potential for future work

==> section/exp.tex <==
\section{Experiments}
\label{sec:exp}
We first evaluate the performance of \chatgpt and LLaMA on five domain-specific either STS or NLI benchmarks, and then measure the predictive confidence and uncertainty over both general, clinical and biomedical domains, followed by assessing the ability of LLMs to make personalised prediction for discriminative NLU tasks.

\subsection{Evaluation Metrics}
\textbf{Accuracy Metrics:} 
For singular values, STS accuracy is generally evaluated with Pearson correlation ($r$) and Spearman rank correlation ($\rho$), measuring the linear correlation between model outputs and the average annotation, the degree of monotonicity under ranking, respectively.
Mean square error (MSE) assesses the models' ability to recover the gold standard. 
For NLI, accuracy and F1-score are used.

However, they only focus on aggregated gold labels: average score and the class type of maximum probability, which is inadequate to evaluate collective distributions and predictive uncertainty.


\textbf{Uncertainty Evaluation Metrics:}
For uncertainty-aware outputs, \ece and \nlpd can be used to assess model reliability in the absence of gold distributions.
\ece measures whether the estimated predictive confidence is aligned with the empirical correctness likelihoods.
A well-calibrated model should be less confident on erroneous predictions and more confident on correct ones.
\nlpd penalises over-confidence more strongly through logarithmic scaling, favouring under-confident models.

With the availability of gold distributions, we apply distributional divergence into the evaluation, to observe the fit between the distribution of collective human judgements and the model predictive probability. 
Following previous work, Kullback-Leibler Divergence (\kl) is used for STS, and \textbf{Jensen-Shannon Distance (JSD)} used for NLI to measure the distance between the softmax multinomial distribution of the models and the distributions over human labels.


\subsection{Results}
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l l l l l}
        \toprule
        Dataset & Personality & $r\uparrow$ & $\rho \uparrow$ & MSE $\downarrow$ \\
        \midrule
        STS-B & Helpful assistant & 0.827 & 0.825 & 1.16 \\
        BIOSSES & Helpful assistant & 0.865 & 0.888 & 0.56 \\
        EBMSASS & Helpful assistant & 0.805 & 0.650 & 0.50 \\
        BIOSSES & Biomedical expert & 0.868 & 0.888 & 0.52 \\
        MedSTS & Helpful assistant & 0.790 & 0.701 & 0.72 \\
        MedSTS & Expert clinician & 0.769 & 0.637 & 0.86 \\
        N2C2-STS & Helpful assistant & 0.817 & 0.754 & 0.90 \\
        N2C2-STS & Expert clinician & 0.765 & 0.742 & 1.53 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Pearson ($r$), Spearman ($\rho$) correlation and MSE of test set over STS datasets across domains under different personality settings as ChatGPT system role.}
    \label{tab:results}
\end{table}


\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l l l l l}
        \toprule
        Model & Accuracy & Prec & Recall & F1-macro \\
        \midrule
        \chatgpt & 0.739 & 0.763 & 0.739 & 0.743 \\
        \vicuna (13B) \\
        \vicuna (7B) \\
        \alpaca (7B) \\
        \bottomrule
    \end{tabular}
    }
    \caption{Accuracy, precision (Prec), recall and F1-macro score on \mednli test set using \chatgpt and open-source LLMs such as \vicuna and \alpaca.}
    \label{tab:mednli}
\end{table}
% chatgpt: {'accuracy': 0.739, 'precision': 0.763, 'recall': 0.739, 'F1': 0.743}


\subsection{Accuracy Evaluation}
We evaluate the performance of \chatgpt, \llama, \alpaca and \vicuna, across five STS and NLI datasets against the aggregated gold labels, by zero-shot and few-shot prompts with and without chain-of-thoughts.
BERT-base
RoBERTa-large

\paragraph{Open-source LLMs} 
We analyse the outputs of \llama, \alpaca and \vicuna (7B parameters) given the same general prompts, and find that responses by \vicuna is the most relevant, meaningful, fluent and coherent, followed by \alpaca, \llama is the least.
This is consistent with the findings in \citet{peng2023vicuna}.
We further evaluate their performance on STS task in zero-shot setting. Similarity scores predicted by \vicuna are always 0.0 even if two sentences are highly similar. This suggests that the prompts we used may be not suitable for \vicuna or the model does not have large capacity to perform well on STS task in zero-shot setting.

We apply \vicuna (13B) over \stsb test set, there are 1.379 example, with only 583 valid predictions.
Pearson correlation 0.545, Spearman correlation 0.516, MSE 1.45

Finish these by the end of this week, it takes too long, and release on arxiv.
Experiment list:
1. vicuna on MedNLI
2. vicuna on USTS-C and USTS-U
3. different prompt strategies on \stsb, \usts and \mednli by \chatgpt, but careful the output format.
4. different roles impact on \usts or \chaosnli


\textbf{Generating in batch affects the generation quality.}
We find that the response by prompting the language model one by one is different from the response generated by batch inference either by padding on the left or on the right, or even without adding ``[PAD]'' token when other inputs are in the same length with the one of interest.



\subsection{Chinese STS corpus}
% impact of language
We evaluated the performance of LLMs over English STS datasets.
Do the language of data impact the accuracy? We evaluate on a Chinese STS corpus --- \usts.
It has two subsets, \ustsc with high human disagreement in labelling and \ustsu with low human disagreement.
For fine-tuned models based on BERT or cosine similarity based on semantic representation of two sentences, it is easier to predict the average score for \ustsu than \ustsc.
That is, higher correlation tends to be achieved on low-disagreement \ustsu.

We have two choices for the language of instructions: English instruction that the LLM is more familiar than other languages, and Chinese instruction that is consistent with the input content.
Will the language of instructions impact the performance?
As shown in \tabref{tab:usts}, over both \ustsc and \ustsu, correlations between the predicted score and the gold label by averaging annotations of all raters are both extremely low (around 0.5), and MSE is large.
This implies that it is challenging for \chatgpt to correctly estimate semantic similarity scores for examples in \usts, either they are high or low human disagreement. 
Using English instruction is better than using Chinese instruction.
% ustsc: 
% zh: Pearson correlation 0.46, Spearman correlation 0.5, MSE 5.0
% en: Pearson correlation 0.56, Spearman correlation 0.55, MSE 2.97
% ustsu: 
% zh: Pearson correlation 0.47, Spearman correlation 0.43, MSE 5.42
% en: Pearson correlation 0.55, Spearman correlation 0.47, MSE 3.09
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l l l l l}
        \toprule
        Dataset & lan\_instruction & $r$ & $\rho$ & MSE \\
        \midrule
        \ustsc (high) & English & 0.556 & 0.551 & 2.97 \\
        \ustsc (high) & Chinese & 0.461 & 0.503 & 5.00 \\
        \ustsu (low) & English & 0.552 & 0.465 & 3.09 \\
        \ustsu (low) & Chinese & 0.472 & 0.435 & 5.42 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Pearson ($r$), Spearman ($\rho$) correlation and MSE of test set over Chinese STS datasets \ustsc (high human disagreement in labelling) and \ustsu (low human disagreement) using \chatgpt helpful assistant role, with instructions (prompts) of two languages: English and Chinese.}
    \label{tab:usts}
\end{table}



\subsection{Uncertainty of }
Based on biomedical STS dataset BIOSSES, we repeat zero-shot experiments 10 times.
As results shown in \figref{fig:biosses-15runs}.

\begin{figure*}[t!]
	\centering
        \includegraphics[scale=0.5]{section/fig/biosses_rp_15_runs.pdf}
	\includegraphics[scale=0.5]{section/fig/biosses_loss_15_runs.pdf}
	\caption{Correlation (left) and MSE loss (right) on biomedical STS: BIOSSES over 15 zero-shot runs using \chatgpt.}
	\label{fig:biosses-15runs}
\end{figure*}



\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l l l c l l l}
        \toprule
        Dataset & Personality & Context & Single-run & $r$ & $\rho$ & MSE \\
        \midrule
        BIOSSES & Helpful assistant & -- & \xmark & 0.874 & 0.892 & 0.50 \\
        BIOSSES & Helpful assistant & -- & \cmark & 0.865 & 0.888 & 0.56 \\
        BIOSSES & Helpful assistant & biomedical & \cmark & 0.871 & 0.877 & 0.53 \\
        BIOSSES & Biomedical expert & -- & \cmark & 0.868 & 0.888 & 0.52 \\
        BIOSSES & Biomedical expert & biomedical & \cmark & 0.848 & 0.865 & 0.61 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Pearson ($r$), Spearman ($\rho$) correlation and MSE on BIOSSES under different personality (system role) and context settings.}
    \label{tab:biossesresults}
\end{table}


how to evaluate the predictive confidence if only accessing to model API? Is it safe and reliable? ChatGPT makes special mechanism to control this, it is good.
how to improve domain performance under LLMs

\textit{Does indicating explicit context in prompt consistently hurt performance?}
Seemingly yes, Why?
check differences for instances where predictions are very different before and after changing the context.


\textbf{With/Without changing system roles, what is the difference?}
Does system role work as it is expected? 
We hypothesise that if assigning system role or explicitly informing LLMs of the domain-specific context in prompt works as it is designed, we expect better performance on biomedical/clinical STS datasets 
Will the uncertainty resulted from sampling be similar to the uncertainty caused by changing system roles?


Our results over STS-B test is:
pearson correlation is 0.8270 and spearman correlation is 0.8253
MSE: 1.16
But we can't compare with the result from \citet{zhong2023can}, as they choose some samples from the uniform similarity distribution, ranging from 0 for no meaning overlap to 5 for meaning equivalence, instead of the whole dev or test set.

\subsection{Results}
Analyse results of biosses:
1. line plot of r and p, if obvious, loss in the same figure: done
2. RQ: Can sampled predictions fit by Gaussian distribution? Is the sampling controlled within a normal distribution?
2. based on the 15 runs, calculate uncertainty metrics results, cal, nlpd, sha, kl with five annotation distribution, and ensemble prediction's r and p
3. RQ: what is the difference between LLM prediction uncertainty and data annotation uncertainty?
draw scatter figure: x is mean and y is std for each example, 100 examples by 100 scatters, one colour for annotation and another colour for prediction.




When we use "You are an expert clinician with rich expertise in medical and clinical domains." as system role, ChatGPT consistently return 
"Thank you for the compliment, but as an AI language model, I don't have personal experience or emotions, and I don't have any opinions or beliefs. However, I have been designed to provide helpful and accurate information on various topics, including medical and clinical domains. How may I assist you today?"



During experiment, we find, same dataset, same persona and prompt, there will be different results. 
Uncertainty stemming from random sampling over different runs in the same setting is different from the uncertainty sourced from inherent human disagreement on STS judgement.
We should distinguish them.

Why we want to evaluate STS and NLI under LLMs in-context learning? What's our expectation for LLMs in traditional NLU tasks? Why we care more and more about models could perform like human beings.
With rapid development of NLP and LLM, we find it really can lead us to compete with humans in accuracy over these tasks, STS and NLI, thus, apart from accuracy, we start to have more demands for current models, for LLMs.

In previous work, we all just hope model to reach the level where it can accurately predict an averaged score, an average opinion for a task, on top of this, we may demanding for robustness and reliability.
But now, when its capability has reached to compete human average level, we hope it could be more intelligent, we hope it can capture more fine-grained features, we hope it could be personalised, instead of group intelligence, not individual intelligence.
We ask: Can powerful LLMs make personalised decision/judgement when it given difference persona?

Previous work show that it will be more toxic when it is given persona of a bad/terrible person, it can also return difference responses if you instruct it to explain to different cohorts, like expert, and five-year old children. 
But these task, either toxic word or explanation in different tone and style, they depend on model's capability of expression, language patterns.
Now, we wonder, if the task not only requires capability of language but reasoning and judgement, can it still make personalised judgement and decision? 
Why it can? Why it can't? if cannot, if we want to move into deep intelligence, personalised modelling, what should we do? A real generative models, that know the joint distribution of how data is generated, joint distribution of input and label.


We have RQ1: over traditional NLU tasks, how uncertain is in-context learning based on LLMs, such as \chatgpt, \gptfour and \bard ?
Where does this uncertainty come from? 
What's the difference of LLMs' prediction uncertainty on NLU tasks from the uncertainty of fine-tuned model?
Is such uncertainty good or bad? What's our expectations for such output? 

Actually, we do not expect always exactly same output for an instance in the same setting, we expect the output vary in a range, this sampling pattern fit a distribution, generally Gaussian distribution, fits human variations in judgement under same context and with similar background knowledge (similar persona).

We should sample 100 examples, or directly use biosses, to evaluate the model uncertainty, or this method uncertainty, using this kind of method, how uncertain it is over STS and NLI tasks?


Now, we have known the uncertainty from model.
Our next RQ: if we change the persona, can LLMs simulate human, and generate personalised output, and the final sampling distribution fit real collective human distribution?
Why it can? or Why it can't?

What's the difference between accuracy relying on language model expression/inertia and the accuracy learned from task-specific tuning (the ability to make decision / judgement)?
change of persona VS change of prompt context? What's the difference between these two?

Above, we will focus on these questions over different datasets, domains and tasks, overall, the change of data under a method, in the next stage of analysis, we will from models and languages to investigate the differences.

In analysis, we can sample some examples, 100 to 200, evaluate over different models, \bard, \chatgpt and \gptfour;
We can analyse languages, that is, we all evaluate English text, there is distribution differences for en and zh, among human annotators, mean, std distribution are different, same for LLMs?



over USTS and chaosNLI datasets.

==> section/method.tex <==
% \section{Method}
% \label{sec:method}

==> section/tables.tex <==
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l | c c c c | c c c c}
        \toprule
        Dataset $\rightarrow$ & \multicolumn{4}{c|}{\stsb} & \multicolumn{4}{c}{\ncsts} \\
        Prompt Strategy $\downarrow$ & \#valid & $r\uparrow$ & $\rho \uparrow$ & MSE $\downarrow$ & \#valid & $r\uparrow$ & $\rho \uparrow$ & MSE $\downarrow$ \\
        \midrule
        zero-shot & 500 & \textbf{0.911} & \textbf{0.899} & \textbf{0.62} & 412 & \textbf{0.817} & \textbf{0.754} & \textbf{0.90} \\
        zero-shot (AG) & 500 & 0.778 & 0.769 & 1.21 & 412 & 0.532 & 0.531 & 2.53 \\
        zero-shot (CoT) & 442 & 0.158 & 0.208 & 7.61 & 368 & 0.173 & 0.185 & 3.75 \\
        \midrule
        % few-shot & 307 & 0.638 & 0.610 & 4.36 & 393 & 0.533 & 0.514 & 3.49 \\
        few-shot & 490 & 0.878 & 0.859 & 0.78 & 393 & 0.533 & 0.514 & 3.49 \\
        % few-shot (AG) & 59 & 0.702 & 0.669 & 1.81 & 389 & 0.505 & 0.469 & 3.03 \\
        few-shot (AG) & 500 & 0.853 & 0.845 & 0.77 & 389 & 0.505 & 0.469 & 3.03 \\
        % few-shot (CoT) & 419 & 0.878 & 0.867 & 1.09 & 412 & 0.637 & 0.680 & 3.18 \\
        few-shot (CoT) & 408 & 0.879 & 0.871 & 1.10 & 412 & 0.637 & 0.680 & 3.18 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Pearson ($r$), Spearman ($\rho$) correlation and MSE of test set over 500 examples in general \stsb and clinical \ncsts test sets using different prompt strategies: AG = with annotation guidelines and CoT = with chain of thought. \#valid = the number of valid responses among 500 examples, where the rest examples are either refued to answer or hard to parse the similarity score in free-style text without by simple rules. }
    \label{tab:promptimpact}
\end{table}


\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l | c c c r | c c c r}
        \toprule
        Dataset $\rightarrow$ & \multicolumn{4}{c|}{\stsb} & \multicolumn{4}{c}{\ncsts} \\
        Prompt Strategy $\downarrow$ & \#valid & $r\uparrow$ & $\rho \uparrow$ & MSE $\downarrow$ & \#valid & $r\uparrow$ & $\rho \uparrow$ & MSE $\downarrow$ \\
        \midrule
        zero-shot & 1379 & 0.017 & 0.087 & 172.98 & 411 & -0.124 & -0.07 & 212.28 \\
        zero-shot (AG) & 1379 & 0.143 & 0.307 & 6.64 & 408 & 0.022 & 0.02 & 117.97 \\
        zero-shot (CoT) & 1379 & 0.066 & 0.142 & 668.74 & 412 & 0.027 & 0.18 & 54.08 \\
        \midrule
        few-shot & 1379 & \textbf{0.528} & \textbf{0.551} & \textbf{3.49} & 412 & \textbf{0.328} & \textbf{0.316} & \textbf{6.99}  \\
        few-shot (AG) & 1379 & 0.397 & 0.378 & 4.46 & 409 & -0.02 & 0.238 & 37.91 \\
        few-shot (CoT) & 1370 & 0.201 & 0.65 & 39.51 & 399 & -0.03 & -0.189 & 635.15 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Pearson ($r$), Spearman ($\rho$) correlation and MSE of full test set in general \stsb and clinical \ncsts test sets using different prompt strategies: AG = with annotation guidelines and CoT = with chain of thought. \#valid = the number of valid responses among 500 examples, where the rest examples are either refused to answer or hard to parse the similarity score in free-style text without by simple rules. }
    \label{tab:llama7b-promptimpact}
\end{table}


\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l | c c c | c c c | c c c }
        \toprule
        Model$\rightarrow$ & \multicolumn{3}{c|}{\textbf{\chatgpt}} & \multicolumn{3}{c|}{\textbf{\llamatwo (7B)}} & \multicolumn{3}{c}{\textbf{\llamatwo (13B)}} \\
        Dataset$\downarrow$ & $r\uparrow$ & F1$\uparrow$ & ECE$\downarrow$ 
        & $r\uparrow$ & F1$\uparrow$ & ECE$\downarrow$ 
        & $r\uparrow$ & F1$\uparrow$ & ECE$\downarrow$ \\
        \midrule
        \medsts & 0.801 & -- &  \textit{0.622} & 0.269 & 0.076 & 0.818 & 0.252 & 0.087 & 0.754 \\
        \biosses & 0.849 & -- & \textit{1.096} & 0.107 & 0.017 & 0.840 & 0.272 & 0.01 & 0.723\\
        \ustsc & 0.809 & -- & \textit{1.442} & -0.124 & 0.114 & 0.0 & -0.179 & 0.122 & 0.0\\
        \midrule
        \mednli & -- & 0.668 & 0.238 -- & 0.312 & 0.457 & -- & 0.407 & 0.277\\
        \chaosnli & -- & 0.541 & 0.215 -- & 0.356 & 0.418 & -- & 0.309 & 0.348\\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{ECE and $r$ and F1 for STS/NLI by \chatgpt and \llamatwo (13B).}
    \label{tab:ece}
\end{table}





